Adversarial confound regression and uncertainty measurements to classify heterogeneous clinical MRI in Mass General Brigham

Automated disease detection in neuroimaging holds promise to improve the diagnostic ability of radiologists, but routinely collected clinical data frequently contains technical and demographic confounding factors that cause data to both differ between sites and be systematically associated with the disease of interest, thus negatively affecting the robustness of diagnostic models. There is a critical need for diagnostic deep learning models that can train on such imbalanced datasets without being influenced by these confounds. In this work, we introduce a novel deep learning architecture, MUCRAN (Multi-Confound Regression Adversarial Network), to train a deep learning model on clinical brain MRI while regressing demographic and technical confounding factors. We trained MUCRAN using 17,076 clinical T1 Axial brain MRIs collected from Massachusetts General Hospital before 2019 and demonstrated that MUCRAN could successfully regress major confounding factors in the vast clinical data. We also applied a method for quantifying uncertainty across an ensemble of these models to automatically exclude out-of-distribution data in the AD detection. By combining MUCRAN and the uncertainty quantification method, we showed consistent and significant increases in the AD detection accuracy for newly collected MGH data (post-2019) and for data from other hospitals. MUCRAN offers a generalizable approach for heterogenous clinical data for deep-learning-based automatic disease detection.

==> GAN Confounds Article/figures/ad_age_acc_comp.tex <==
\begin{figure}[!h]
\centering
%\includegraphics[width=0.30\textwidth]{images/grad_cam_unconfounded.png}
%\includegraphics[width=0.30\textwidth]{images/grad_cam_confounded.png}
{\sffamily
\centering
\includegraphics[width=0.8\textwidth]{images/ad_age_acc_comp_post.png}
}
\caption{{\bf Comparison of classification accuracies on post-2019 data for an age-matched sample of patients aged 55 and older in MGH, BWH, and outside hospital datasets.}
A. Results in the internal, post-2019 MGH test set. B. Results on post-2019 data from Brigham and Women's Hospital. C. Results from all outside hospital systems imported into Mass General Brigham. See Table \ref{tab:results_alz} for the full results.}
\label{fig:ad_age_acc_comp}
\end{figure}

==> GAN Confounds Article/figures/cam_results.tex <==
\begin{figure}[t!]
\centering
%\includegraphics[width=0.30\textwidth]{images/grad_cam_unconfounded.png}
%\includegraphics[width=0.30\textwidth]{images/grad_cam_confounded.png}
{\sffamily
\centering
\includegraphics[width=0.8\textwidth]{images/brain_mesh_perc.png}
}
\caption{\textbf{Averaged gradient class activation map results.} A. Gradient-weighted class activation mapping (Grad-CAM) results for confounded and regressed models, thresholded at 0.15. The regressed model, in which compounding factors were regressed, shows higher activations inside the brain than the confounded model. B. A 3D mesh representation of the Grad-CAM data; a glass brain (in red) is included for visualization purposes. C. Total voxels in each ensemble covering the middle (brain) and edge areas.}
\label{fig:cam_results}
\end{figure}

==> GAN Confounds Article/figures/confounds_diagram.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=0.8\textwidth]{images/confound_auroc.png}

\caption{{\bf Prediction of confounding factors.}
Averaged results of model performance for predicting demographic and technical confounding factors were reported as area under the receiver operating characteristics (AUROC) for the confounded and regressed ensembles.}
\label{fig:confounds_diagram}
\end{figure}

==> GAN Confounds Article/figures/dataset_description.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=0.90\textwidth]{images/dataset_description_ages.png}
\caption{{\bf Statistics associated with the three datasets used, pre- and post-2019.}
T1 Axial MRI, representing the plurality of structural MRI in the Mass General Brigham database, were taken from our full database of imaging data, and, from these, three test sets were isolated. "Local anomaly" refers to patients with lesions, head trauma, or tumors. The average age and standard deviation of each group is shown as well.}
\label{fig:dataset_description}
\end{figure}

==> GAN Confounds Article/figures/gan_pipeline_fig.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=0.80\textwidth]{images/gan_pipeline_fig_layout.png}
\caption{{\bf Multi-Confound Regression Adversarial Network (MUCRAN).}
A. MUCRAN is a convolutional neural network (CNN) that takes a $96\times 96\times 96$ MRI as input, encodes it to an array of 1024 intermediary features via a CNN and a dense neural network, and regresses these features to an output array. The output array consists of one-hot binary vectors that encode both the primary label (AD/Control) and included confounding factors (sex, age, and so on). B. For training the regressed model, large batches are sampled from an imbalanced dataset such that AD and control are present in equal proportions. For each training iteration, the model is trained in a two-step adversarial process: with the regressor frozen, the encoder is fit to an output array with the label set to its real value, but each confound row set to a constant value ($[1,0,0...0]$); the regressor is then fit to the array with both the label and its true confound values. C. For testing, labels are predicted through multiple independent models, and their votes are averaged into an ensemble vote. An uncertainty thresholding is then applied to isolate an in-distribution test set.}
\label{fig:gan_pipeline_fig}
\end{figure}

==> GAN Confounds Article/figures/loss.tex <==
\begin{figure}[t!]
\centering
{\sffamily
\includegraphics[width=0.80\textwidth]{images/gan_pipeline_layout.png}

%\begin{tabular}{ccc}
%& \textbf{Regressor} & \textbf{Encoder} \\
%\put(0,0){\rotatebox{90}{\phantom{00000000000000}\textbf{}}}  & \includegraphics[width=0.45\textwidth]{images/encoder_loss.png} & \includegraphics[width=0.45\textwidth]{images/regressor_loss.png}
%\end{tabular}
}

\caption{A. The model used is a CNN that takes a $96\times 96 \times 96$ MRI as input, encodes it to an array of 1024 intermediary features via a CNN and a dense neural network, and regresses these features to an output array. The output array consists of one-hot binary vectors that encode both the primary label (AD/Control) and included confounds (Sex, Age, and so on). B. For training the regressed model, large batches are sampled from an imbalanced dataset such that AD and Control are present in equal proportions. For each training iteration, the model is trained in two-step adversarial process: with the regressor frozen, the encoder is fit to an output array with the label set to its real value, but each confound row set to a constant value ([1,0,0...0]); the regressor is then fit to the array with both the label and its true confound values. C. For testing, labels are predicted through multiple independent models, and their votes are averaged into an ensemble vote. The maximum averaged vote is guaranteed to exceed 0.5, and so that is included in the whole test set; however, a subset of this is also evaluated based on whether or not this averaged vote exceeds a higher threshold. See also Table \ref{tab:results_table}.}
\label{fig:gan_pipeline_fig}
\end{figure}

==> GAN Confounds Article/figures/moving_window_auroc.tex <==
\begin{figure}[t!]
\begin{tabular}{cccc}
& \textbf{MGH (post-2019)} & \textbf{BWH} & \textbf{Other} \\
\put(0,0){\rotatebox{90}{\phantom{00000000000}\textbf{}}}  & \includegraphics[width=0.3\textwidth]{images/Ages_mgh.png} & \includegraphics[width=0.3\textwidth]{images/Ages_bwh.png} &
\includegraphics[width=0.3\textwidth]{images/Ages_other.png}
\end{tabular}

\caption{\textbf{}}
\label{fig:confounds_diagram}
\end{figure}

==> GAN Confounds Article/figures/test_set_anatomy.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{images/test_anatomy_fig_55.png}

\caption{\textbf{Anatomy of a test set, showing the two critical contributions of this work.} This shows, for Alzheimer's classification, the test set divided into three cases: out-of-distribution data, in which data is too unlike training data to make any determination; indeterminate cases, in which the case may be in-distribution but not be a clear-cut case of Alzheimer's or control; and in-distribution data, in which all models in the ensemble agree on a classification. The age intersection between AD and Control cases show the cases for which MUCRAN performed significantly better than the confounded or baseline comparisons.}
\label{fig:test_set_anatomy}
\end{figure}

==> GAN Confounds Article/figures/uncertainty_plots.tex <==
\begin{figure}[t!]
\centering

{\sffamily
\begin{tabular}{ccc}
 \textbf{Confounded} & \textbf{No Confounds} & \textbf{Regressed}\\
 \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_converg_hist_PatientID.png}
 & \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_dud_hist_PatientID.png} &
 \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_hist_PatientID.png}
\end{tabular} \\
\begin{tabular}{cc}
 \textbf{Distribution Comparison} & \textbf{Accuracy Comparison} \\
 \includegraphics[height=0.36\textwidth]{images/hist_lines_PatientID.png} &
 \includegraphics[height=0.36\textwidth]{images/uncertainty_plots_PatientID.png}
\end{tabular}

}

\caption{\textbf{Accuracies for ensemble predictions with different test set inclusion thresholds.} The histograms show the distribution of values in the regressed (top) and confounded (bottom) ensembles. The graphs show the same data, but explicitly in terms of accuracy, when data below a given threshold is removed. Regressed models offer greater stability and certainty for a larger portion of the data than confounded models.}
\label{fig:uncertainty_plots}
\end{figure}

==> GAN Confounds Article/figures/uncertainty_plots2.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.30\textwidth]{images/grad_cam_unconfounded.png}
%\includegraphics[width=0.30\textwidth]{images/grad_cam_confounded.png}
{\sffamily
\begin{tabular}{cccc}
& \textbf{MGH} & \textbf{BWH} & \textbf{Other} \\
\put(0,0){\rotatebox{90}{\phantom{00000000}\textbf{Before 2019}}}  & {} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_bwh_before_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_other_before_2019.png} \\
\put(0,0){\rotatebox{90}{\phantom{00000000}\textbf{After 2019}}}  & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_mgh_after_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_bwh_after_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_other_after_2019.png}
\end{tabular}
}
\caption{\textbf{Relative accuracy of each ensemble in threshold values between 0.00 and 0.99.} Lines on these graphs show the intermediate accuracies and number of included datapoints in each test set for values between 0.00 and 0.99; see table \ref{tab:results_table}.}
\label{fig:uncertainty_plots2}
\end{figure}

==> GAN Confounds Article/tables/confounds_predictions.tex <==
\begin{table}[b!]
\centering
\caption{Averaged results of the confounds (AUCs) for both the regressed and confounded models.}
\label{tab:confounds_predictions}
\sffamily
\begin{tabular}{lrr}
\toprule
Confound Name &  Confounded Model AUROC & Regressed Model AUROC \\
\midrule
Ages                &    0.644080 &   0.544823 \\
EchoTime            &    0.000000 &   0.000000 \\
Employment Status &    0.568977 &   0.502733 \\
Ethnic Group      &    0.537599 &   0.498418 \\
Imaging Frequency    &    0.790025 &   0.472857 \\
Marital Status   &    0.545788 &   0.507806 \\
Patient Class      &    0.577736 &   0.484328 \\
Pixel Bandwidth      &    0.666692 &   0.493821 \\
Religion         &    0.509234 &   0.488828 \\
Repetition Time      &    0.615542 &   0.486065 \\
Specific Absorption Rate                 &    0.670172 &   0.493353 \\
Sex               &    0.849446 &   0.447886 \\
Slice Thickness      &    0.000000 &   0.000000 \\
\bottomrule
\end{tabular}
\end{table}


==> GAN Confounds Article/tables/dataset_description.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\sffamily
\begin{tabular}{l|rr|rr|rr}
\toprule
{} & AD (MGH pre-2019) & Control (MGH pre-2019) & AD (BWH pre-2019) & Control (BWH pre-2019) & AD (Other pre-2019) & CONTROL (Other pre-2019) \\
\midrule
No. Males & 1778 & 5657 & 1810 & 3594 & 221 & 458 \\
No. Females & 2435 & 6951 & 2420 & 5476 & 409 & 848 \\
Age (mean±std) & 722.23 ± 169.55 & 471.82 ± 191.53 & 695.34 ± 172.58 & 504.44 ± 167.14 & 714.34 ± 187.04 & 488.27 ± 166.62 \\
Unique Patient IDs & 1060 & 4215 & 1023 & 2986 & 251 & 520 \\
Slice Thickness & 4.59 ± 0.88 & 4.33 ± 1.04 & 3.93 ± 1.18 & 3.84 ± 1.11 & 3.83 ± 1.49 & 4.11 ± 1.19 \\
No. Unique Datapoints & 4213 & 12608 & 4230 & 9070 & 630 & 1306 \\
No. Unique Sites & 37 & 42 & 38 & 38 & 97 & 211 \\
Echo Time & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 \\
Repetition Time & 0.55 ± 0.34 & 0.55 ± 0.32 & 0.59 ± 0.29 & 0.59 ± 0.25 & 0.72 ± 0.52 & 0.59 ± 0.36 \\
Specific Absorption Rate & 0.79 ± 0.59 & 0.79 ± 0.64 & 0.72 ± 0.59 & 0.71 ± 0.54 & 0.58 ± 0.49 & 0.70 ± 0.52 \\
Imaging Frequency & 79.71 ± 26.71 & 77.25 ± 25.51 & 81.18 ± 27.55 & 74.34 ± 23.10 & 86.61 ± 29.26 & 81.68 ± 28.06 \\
Pixel Bandwidth & 161.83 ± 77.45 & 149.96 ± 72.58 & 162.42 ± 100.59 & 141.88 ± 71.64 & 201.59 ± 110.49 & 177.18 ± 101.74 \\
No. Unique Religions & 30 & 37 & 30 & 30 & 19 & 27 \\
No. Unique Ethnicities & 5 & 7 & 5 & 7 & 5 & 6 \\
\midrule
{} & AD (MGH post-2019) & Control (MGH post-2019) & AD (BWH post-2019) & Control (BWH post-2019) & AD (Other post-2019) & CONTROL (Other post-2019) \\
\midrule
No. Males & 143 & 529 & 229 & 426 & 58 & 207 \\
No. Females & 211 & 584 & 281 & 595 & 104 & 314 \\
Age (mean±std) & 754.04 ± 176.39 & 552.07 ± 171.99 & 816.87 ± 159.84 & 519.20 ± 186.70 & 794.06 ± 142.25 & 511.45 ± 173.74 \\
Unique Patient IDs & 131 & 461 & 207 & 438 & 84 & 232 \\
Slice Thickness & 4.17 ± 1.30 & 3.92 ± 1.29 & 3.24 ± 1.59 & 2.73 ± 1.51 & 4.24 ± 1.34 & 3.79 ± 1.58 \\
No. Unique Datapoints & 354 & 1113 & 510 & 1021 & 162 & 521 \\
No. Unique Sites & 17 & 18 & 18 & 23 & 30 & 75 \\
Echo Time & 0.02 ± 0.02 & 0.02 ± 0.02 & 0.01 ± 0.00 & 0.01 ± 0.00 & 0.01 ± 0.00 & 0.01 ± 0.00 \\
Repetition Time & 1.06 ± 0.84 & 0.98 ± 0.80 & 0.88 ± 0.64 & 0.93 ± 0.74 & 0.71 ± 0.49 & 0.63 ± 0.50 \\
Specific Absorption Rate & 0.66 ± 0.49 & 0.64 ± 0.50 & 0.37 ± 0.36 & 0.35 ± 0.36 & 0.85 ± 0.54 & 0.80 ± 0.63 \\
Imaging Frequency & 90.58 ± 30.61 & 87.66 ± 30.35 & 99.91 ± 29.37 & 105.22 ± 34.30 & 82.07 ± 27.54 & 80.00 ± 26.68 \\
Pixel Bandwidth & 249.56 ± 102.89 & 236.10 ± 110.17 & 253.09 ± 109.79 & 258.53 ± 102.76 & 171.41 ± 92.82 & 161.73 ± 77.02 \\
No. Unique Religions & 21 & 25 & 21 & 24 & 12 & 14 \\
No. Unique Ethnicities & 5 & 6 & 3 & 5 & 3 & 5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Statistics associated with the three datasets used. The model in this paper was trained on the pre-2019 MGH data. Shown for continuous values are the mean and standard deviations. \label{tab:dataset_description}}
\end{table}

==> GAN Confounds Article/tables/methods_comparison_table.tex <==
\begin{table}[!h]
\sffamily
\caption{Comparison of MUCRAN with other generalizable variable regression methods used in neuroimaging}
\begin{adjustbox}{width=0.80\textwidth,totalheight=0.80\textheight,keepaspectratio}

\begin{tabular}{p{5cm}|lllp{5cm}p{2cm}}
Regression Method & Multivariate? & Hand-crafted features? & Affects training set size & Notes & References \\ \hline
Confounder-Free DL Model & No & No & No & In early tests, attempts to apply multivariate regression led to mode collapse. & \cite{Zhao2020} \\
Data Matching & Yes & No & Yes & & \cite{Leming2022}  \\
Post-Hoc Counterbalancing & No & No & Yes & & \cite{Snoek2019}  \\
Regression of extracted features & Yes & Yes & No & Refers to a class of methods, such as ComBat and Linear Mixed-Effects Models, that require significant feature reduction/extraction and treat features as independent scalar components, as images are too high-dimensional for these methods to work on them directly. The exact method of feature reduction varies between studies. & \cite{Johnson2007,Bolker2009,Todd2013,Kostro2014,Dubois2018,EspinPerez2018,Yu2018,Snoek2019,More2021} \\
\hline
MUCRAN & Yes & No & No & & Current Work \\
\end{tabular}
\end{adjustbox}
\label{tab:methods_comparison_table}
\end{table}


==> GAN Confounds Article/tables/results_alz.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results on Alzheimer's classification when the whole test set is included (threshold = 0.5), and results, on five test sets and the combined test sets, for which the averaged prediction in its respective category is above 0.90 (i.e., each model in the ensemble unanimously agrees). Shown are the accuracies on the portion of the dataset included after thresholding, and the size of that test set (in parentheses). Included as well are age-matched samples. See also Figure \ref{fig:gan_pipeline_fig}C.}

\label{tab:results_alz}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{l|}{\multirow{12}{*}{Alzheimer’s}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{92.5\% (548)} & \textbf{89.2\% (3721)} & \textbf{93.5\% (367)} & \textbf{92.1\% (643)} & \textbf{90.5\% (285)} & \textbf{89.1\% (5783)} \\
\multicolumn{1}{l|}{} & & & Baseline & 87.7\% (778) & 84.4\% (6198) & 89.8\% (637) & 88.4\% (976) & 91.0\% (390) & 84.7\% (9469) \\
\multicolumn{1}{l|}{} & & & Confounded & 89.5\% (829) & 84.1\% (7265) & 87.6\% (740) & 86.3\% (1138) & 90.5\% (419) & 83.9\% (10951) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 75.8\% (1463) & 72.4\% (13303) & 75.2\% (1531) & \textbf{76.9\% (1936)} & 80.2\% (681) & 72.1\% (20857) \\
\multicolumn{1}{l|}{} & & & Baseline & 77.4\% (1463) & \textbf{72.9\% (13303)} & \textbf{76.3\% (1531)} & 74.7\% (1936) & \textbf{81.6\% (681)} & \textbf{72.4\% (20857)} \\
\multicolumn{1}{l|}{} & & & Confounded & \textbf{78.4\% (1463)} & \textbf{72.9\% (13303)} & 74.7\% (1531) & 74.7\% (1936) & 81.2\% (681) & 72.3\% (20857) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Age-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{86.0\% (150)} & \textbf{67.0\% (880)} & \textbf{77.3\% (44)} & \textbf{73.5\% (166)} & \textbf{71.9\% (32)} & \textbf{70.1\% (1516)} \\
\multicolumn{1}{l|}{} & & & Baseline & 71.6\% (222) & 57.7\% (1962) & 66.4\% (110) & 65.3\% (314) & 65.8\% (76) & 60.8\% (3064) \\
\multicolumn{1}{l|}{} & & & Confounded & 71.1\% (228) & 54.6\% (2452) & 59.1\% (164) & 60.1\% (376) & 54.3\% (70) & 56.6\% (3846) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & \textbf{65.2\% (494)} & \textbf{56.7\% (6372)} & 55.6\% (446) & \textbf{60.7\% (746)} & \textbf{66.7\% (168)} & \textbf{58.3\% (10264)} \\
\multicolumn{1}{l|}{} & & & Baseline & 64.8\% (494) & 56.6\% (6372) & \textbf{57.8\% (446)} & 57.1\% (746) & 65.5\% (168) & 57.6\% (10264) \\
\multicolumn{1}{l|}{} & & & Confounded & 64.2\% (494) & 55.2\% (6372) & 55.2\% (446) & 55.9\% (746) & 59.5\% (168) & 56.7\% (10264) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> GAN Confounds Article/tables/results_alz_55.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[!h]
\caption{Results on Alzheimer's classification when the whole test set is included (threshold = 0.5), and results, on five test sets and the combined test sets, for which the averaged prediction in its respective category is above 0.90 (i.e., each model in the ensemble unanimously agrees). Shown are the accuracies on the portion of the dataset included after thresholding, and the size of that test set (in parentheses). Included as well are age-matched samples. See also Figure \ref{fig:gan_pipeline_fig}C.}

\label{tab:results_alz}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{l|}{\multirow{12}{*}{Alzheimer’s}} & \multirow{6}{*}{\parbox{2cm}{Age-matched sample (age 55+)}} & \multirow{3}{*}{0.90 (In-distribution)} & MUCRAN & \textbf{84.6\% (117)} & \textbf{75.4\% (471)} & \textbf{90.3\% (31)} & \textbf{90.9\% (66)} & \textbf{81.0\% (21)} & \textbf{75.3\% (857)} \\
\multicolumn{1}{l|}{} &  &  & Baseline & 72.5\% (160) & 65.4\% (771) & 71.9\% (64) & 75.7\% (181) & 71.0\% (62) & 67.4\% (1317) \\
\multicolumn{1}{l|}{} &  &  & Confounded & 72.3\% (166) & 59.6\% (971) & 62.5\% (104) & 66.5\% (179) & 56.4\% (55) & 61.8\% (1655) \\ \cline{3-10} 
\multicolumn{1}{l|}{} &  & \multirow{3}{*}{0.50 (All data)} & MUCRAN & \textbf{64.9\% (276)} & 57.0\% (2923) & 55.3\% (293) & \textbf{60.3\% (315)} & 63.1\% (141) & \textbf{58.1\% (4776)} \\
\multicolumn{1}{l|}{} &  &  & Baseline & 63.3\% (275) & \textbf{57.5\% (2923)} & 56.5\% (299) & 55.3\% (311) & 64.3\% (140) & 57.9\% (4699) \\
\multicolumn{1}{l|}{} &  &  & Confounded & 63.4\% (276) & 55.9\% (2929) & \textbf{56.6\% (309)} & 55.4\% (316) & \textbf{66.2\% (142)} & 57.2\% (4698) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90 (In-distribution)} & MUCRAN & \textbf{92.5\% (548)} & \textbf{89.2\% (3721)} & \textbf{93.5\% (367)} & \textbf{92.1\% (643)} & \textbf{90.5\% (285)} & \textbf{89.1\% (5783)} \\
\multicolumn{1}{l|}{} & & & Baseline & 87.7\% (778) & 84.4\% (6198) & 89.8\% (637) & 88.4\% (976) & 91.0\% (390) & 84.7\% (9469) \\
\multicolumn{1}{l|}{} & & & Confounded & 89.5\% (829) & 84.1\% (7265) & 87.6\% (740) & 86.3\% (1138) & 90.5\% (419) & 83.9\% (10951) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50 (All data)} & MUCRAN & 75.8\% (1463) & 72.4\% (13303) & 75.2\% (1531) & \textbf{76.9\% (1936)} & 80.2\% (681) & 72.1\% (20857) \\
\multicolumn{1}{l|}{} & & & Baseline & 77.4\% (1463) & \textbf{72.9\% (13303)} & \textbf{76.3\% (1531)} & 74.7\% (1936) & \textbf{81.6\% (681)} & \textbf{72.4\% (20857)} \\
\multicolumn{1}{l|}{} & & & Confounded & \textbf{78.4\% (1463)} & \textbf{72.9\% (13303)} & 74.7\% (1531) & 74.7\% (1936) & 81.2\% (681) & 72.3\% (20857) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> GAN Confounds Article/tables/results_local.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results for localized anomaly classifications, as well as a site-matched sample.}

\label{tab:results_local}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{p{2cm}|}{\multirow{12}{*}{\parbox{2cm}{Ischemia/ Lesion/ Tumor/ Head Trauma}}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & 74.9\% (521) & 80.5\% (2918) & 65.1\% (763) & 65.8\% (803) & 59.4\% (229) & 75.9\% (6783) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{76.2\% (564)} & \textbf{82.3\% (3452)} & \textbf{71.5\% (820)} & \textbf{72.9\% (893)} & \textbf{71.8\% (252)} & \textbf{79.5\% (7891)} \\
\multicolumn{1}{l|}{} & & & Confounded & 73.6\% (754) & 78.8\% (5177) & 66.8\% (1025) & 67.1\% (1217) & 64.3\% (367) & 75.3\% (10500) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 63.2\% (2421) & 68.1\% (19786) & 61.1\% (3558) & 62.5\% (3780) & 62.6\% (1276) & 66.2\% (35264) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{63.9\% (2421)} & \textbf{68.7\% (19786)} & \textbf{61.7\% (3558)} & \textbf{64.5\% (3780)} & \textbf{62.7\% (1276)} & \textbf{67.1\% (35264)} \\
\multicolumn{1}{l|}{} & & & Confounded & 63.5\% (2421) & 68.4\% (19786) & 60.5\% (3558) & 62.1\% (3780) & 60.7\% (1276) & 66.1\% (35264) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Site-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{72.3\% (368)} & 71.8\% (1486) & \textbf{74.4\% (238)} & 64.3\% (196) & 60.7\% (84) & 70.0\% (2658) \\
\multicolumn{1}{l|}{} & & & Baseline & 71.8\% (358) & \textbf{74.7\% (1670)} & 73.0\% (196) & \textbf{73.1\% (208)} & \textbf{69.7\% (66)} & \textbf{70.7\% (2858)} \\
\multicolumn{1}{l|}{} & & & Confounded & 70.2\% (530) & 69.9\% (2774) & 73.2\% (410) & 67.6\% (306) & 59.0\% (100) & 68.8\% (4570) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 61.6\% (2028) & 64.7\% (11926) & 62.3\% (1848) & \textbf{64.4\% (1198)} & 59.2\% (424) & 63.7\% (19514) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{61.9\% (2028)} & \textbf{65.0\% (11926)} & 61.2\% (1848) & \textbf{64.4\% (1198)} & \textbf{62.7\% (424)} & 63.6\% (19514) \\
\multicolumn{1}{l|}{} & & & Confounded & 61.6\% (2028) & 64.9\% (11926) & \textbf{63.9\% (1848)} & 63.5\% (1198) & 59.4\% (424) & \textbf{63.9\% (19514)} \end{tabular}
\end{adjustbox}
\end{table}


==> GAN Confounds Article/tables/results_sex.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[!h]
\caption{Results for sex classification}

\label{tab:results_sex}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{2}{l|}{\multirow{6}{*}{Sex}} & \multirow{3}{*}{0.90 (In-distribution)} & MUCRAN & 96.0\% (1293) & \textbf{96.8\% (11834)} & \textbf{96.3\% (1789)} & \textbf{96.8\% (2345)} & \textbf{97.2\% (723)} & \textbf{96.1\% (18836)} \\
\multicolumn{2}{l|}{} & & Baseline & 96.1\% (1279) & 94.6\% (11619) & 92.7\% (1716) & 95.5\% (2277) & 95.8\% (689) & 93.7\% (18422) \\
\multicolumn{2}{l|}{} & & Confounded & \textbf{96.5\% (1304)} & 96.0\% (11380) & 95.5\% (1782) & 96.5\% (2335) & 97.2\% (712) & 95.5\% (18327) \\ \cline{3-10} 
\multicolumn{2}{l|}{} & \multirow{3}{*}{0.50 (All data)} & MUCRAN & \textbf{85.6\% (2789)} & \textbf{85.7\% (24022)} & \textbf{83.9\% (4083)} & 87.2\% (4427) & \textbf{87.4\% (1444)} & \textbf{85.7\% (36765)} \\
\multicolumn{2}{l|}{} & & Baseline & 85.1\% (2789) & 80.1\% (24022) & 79.4\% (4083) & 84.7\% (4427) & 83.4\% (1444) & 81.7\% (36765) \\
\multicolumn{2}{l|}{} & & Confounded & 85.5\% (2789) & 85.2\% (24022) & 83.1\% (4083) & \textbf{87.4\% (4427)} & 86.6\% (1444) & 85.3\% (36765) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> GAN Confounds Article/tables/results_table.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t]
\caption{Results when the whole test set is included, and results for which the averaged prediction in its respective category is above 0.99 (i.e., each model in the ensemble unanimously agrees).}

\label{tab:results_table}
\sffamily
\begin{tabular}{rllrrrrr}
\toprule
\multirow{2}{*}{Threshold} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{MGH} & \multicolumn{2}{c|}{BWH} & \multicolumn{2}{c|}{Others} \\
 & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} \\ \hline
0.99 & \multirow{2}{*}{Regressed} & Accuracy & 92.2 & 86.3 & 91.5 & 89.5 & 95.2 \\
 & & No. Included Datapoints & 628 & 5297 & 539 & 848 & 335 \\
 & \multirow{2}{*}{Confounded} & Accuracy & 88.8 & 85.5 & 90.0 & 88.0 & 92.1 \\
 & & No. Included Datapoints & 760 & 6565 & 671 & 1031 & 382 \\
 & \multirow{2}{*}{Label Only} & Accuracy & 89.3 & 84.2 & 88.8 & 86.3 & 92.6 \\
 & & No. Included Datapoints & 836 & 6829 & 695 & 1065 & 417 \\ \hline
0.50 & \multirow{2}{*}{Regressed} & Accuracy & 76.2 & 73.2 & 75.8 & 75.7 & 81.2 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
 & \multirow{2}{*}{Confounded} & Accuracy & 78.5 & 73.4 & 75.2 & 75.9 & 82.5 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
 & \multirow{2}{*}{Label Only} & Accuracy & 78.9 & 72.7 & 75.0 & 75.2 & 81.6 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\bottomrule
\end{tabular}
\end{table}


==> GAN Confounds Article/tables/results_table_unthresholded.tex <==
\begin{table}[]
\caption{Results when all data are included (i.e., no threshold).}
\label{tab:results_table_unthresholded}
\begin{tabular}{lllllll}
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{MGH} & \multicolumn{2}{c|}{BWH} & \multicolumn{2}{c|}{Others} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} \\ \hline
\multirow{2}{*}{Regressed} & Accuracy & 76.2 & 73.2 & 75.8 & 75.7 & 81.2 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\multirow{2}{*}{Confounded} & Accuracy & 78.5 & 73.4 & 75.2 & 75.9 & 82.5 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\multirow{2}{*}{No confounds} & Accuracy & 78.9 & 72.7 & 75.0 & 75.2 & 81.6 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 
\end{tabular}
\end{table}

==> GAN Confounds Article/tables/results_tablev2.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t]
\caption{Results when the whole test set is included, and results for which the averaged prediction in its respective category is above 0.99 (i.e., each model in the ensemble unanimously agrees).}

\label{tab:results_table}
\sffamily
\begin{tabular}{lllllll|l}
\multirow{2}{*}{Threshold} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{MGH}       & \multicolumn{2}{c|}{BWH}                                       & \multicolumn{2}{c|}{Others}                      & \multicolumn{1}{l|}{\textbf{All}} \\
                           & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019        & \multicolumn{1}{l|}{\textbf{}}    \\ \hline
0.99                       & Regressed                                    & 92.2\% (628/1467)              & 86.3\% (5297/13300)           & 91.5\% (539/1531)              & 89.5\% (848/1936)             & 95.2\% (335/683) & \textbf{86.9\% (7958/20860)}      \\
                           & Confounded                                   & 88.8\% (760/1467)              & 85.5\% (6565/13300)           & 90.0\% (671/1531)              & 88.0\% (1031/1936)            & 92.1\% (382/683) & \textbf{85.3\% (9892/20860)}      \\
                           & Label only                                   & 89.3\% (836/1467)              & 84.2\% (6829/13300)           & 88.8\% (695/1531)              & 86.3\% (1065/1936)            & 92.6\% (417/683) & \textbf{84.3\% (10374/20860)}     \\ \hline
0.00                       & Regressed                                    & 76.2\% (1467/1467)             & 73.2\% (13300/13300)          & 75.8\% (1531/1531)             & 75.7\% (1936/1936)            & 81.2\% (683/683) & \textbf{72.7\% (20860/20860)}     \\
                           & Confounded                                   & 78.5\% (1467/1467)             & 73.4\% (13300/13300)          & 75.2\% (1531/1531)             & 75.9\% (1936/1936)            & 82.5\% (683/683) & \textbf{72.8\% (20860/20860)}     \\
                           & Label only                                   & 78.9\% (1467/1467)             & 72.7\% (13300/13300)          & 75.0\% (1531/1531)             & 75.2\% (1936/1936)            & 81.6\% (683/683) & \textbf{72.3\% (20860/20860)}    
\end{tabular}

\end{table}


==> GAN Confounds Article/tables/results_tablev3.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results when the whole test set is included (threshold = 0.5), and results for which the averaged prediction in its respective category is above 0.90 (i.e., each model in the ensemble unanimously agrees). Shown are the accuracies on the portion of the dataset included after thresholding, and the size of that test set (in parentheses). Included as well are age-matched samples of the Alzheimer's classification and site-matched samples of localized anomaly classifications. See also Figure \ref{fig:gan_pipeline_fig} C.}

\label{tab:results_table}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{l|}{\multirow{12}{*}{Alzheimer’s}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{92.5\% (548)} & \textbf{89.2\% (3721)} & \textbf{93.5\% (367)} & \textbf{92.1\% (643)} & \textbf{90.5\% (285)} & \textbf{89.1\% (5783)} \\
\multicolumn{1}{l|}{} & & & Baseline & 87.7\% (778) & 84.4\% (6198) & 89.8\% (637) & 88.4\% (976) & 91.0\% (390) & 84.7\% (9469) \\
\multicolumn{1}{l|}{} & & & Confounded & 89.5\% (829) & 84.1\% (7265) & 87.6\% (740) & 86.3\% (1138) & 90.5\% (419) & 83.9\% (10951) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 75.8\% (1463) & 72.4\% (13303) & 75.2\% (1531) & \textbf{76.9\% (1936)} & 80.2\% (681) & 72.1\% (20857) \\
\multicolumn{1}{l|}{} & & & Baseline & 77.4\% (1463) & \textbf{72.9\% (13303)} & \textbf{76.3\% (1531)} & 74.7\% (1936) & \textbf{81.6\% (681)} & \textbf{72.4\% (20857)} \\
\multicolumn{1}{l|}{} & & & Confounded & \textbf{78.4\% (1463)} & \textbf{72.9\% (13303)} & 74.7\% (1531) & 74.7\% (1936) & 81.2\% (681) & 72.3\% (20857) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Age-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{86.0\% (150)} & \textbf{67.0\% (880)} & \textbf{77.3\% (44)} & \textbf{73.5\% (166)} & \textbf{71.9\% (32)} & \textbf{70.1\% (1516)} \\
\multicolumn{1}{l|}{} & & & Baseline & 71.6\% (222) & 57.7\% (1962) & 66.4\% (110) & 65.3\% (314) & 65.8\% (76) & 60.8\% (3064) \\
\multicolumn{1}{l|}{} & & & Confounded & 71.1\% (228) & 54.6\% (2452) & 59.1\% (164) & 60.1\% (376) & 54.3\% (70) & 56.6\% (3846) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & \textbf{65.2\% (494)} & \textbf{56.7\% (6372)} & 55.6\% (446) & \textbf{60.7\% (746)} & \textbf{66.7\% (168)} & \textbf{58.3\% (10264)} \\
\multicolumn{1}{l|}{} & & & Baseline & 64.8\% (494) & 56.6\% (6372) & \textbf{57.8\% (446)} & 57.1\% (746) & 65.5\% (168) & 57.6\% (10264) \\
\multicolumn{1}{l|}{} & & & Confounded & 64.2\% (494) & 55.2\% (6372) & 55.2\% (446) & 55.9\% (746) & 59.5\% (168) & 56.7\% (10264) \\ \hline
\multicolumn{1}{p{2cm}|}{\multirow{12}{*}{\parbox{2cm}{Ischemia/ Lesion/ Tumor/ Head Trauma}}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & 74.9\% (521) & 80.5\% (2918) & 65.1\% (763) & 65.8\% (803) & \textbf{59.4\% (229)} & 75.9\% (6783) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{76.2\% (564)} & \textbf{82.3\% (3452)} & \textbf{71.5\% (820)} & \textbf{72.9\% (893)} & \textbf{71.8\% (252)} & \textbf{79.5\% (7891)} \\
\multicolumn{1}{l|}{} & & & Confounded & 73.6\% (754) & 78.8\% (5177) & 66.8\% (1025) & 67.1\% (1217) & 64.3\% (367) & 75.3\% (10500) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 63.2\% (2421) & 68.1\% (19786) & 61.1\% (3558) & 62.5\% (3780) & 62.6\% (1276) & 66.2\% (35264) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{63.9\% (2421)} & \textbf{68.7\% (19786)} & \textbf{61.7\% (3558)} & \textbf{64.5\% (3780)} & \textbf{62.7\% (1276)} & \textbf{67.1\% (35264)} \\
\multicolumn{1}{l|}{} & & & Confounded & 63.5\% (2421) & 68.4\% (19786) & 60.5\% (3558) & 62.1\% (3780) & 60.7\% (1276) & 66.1\% (35264) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Site-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{72.3\% (368)} & 71.8\% (1486) & \textbf{74.4\% (238)} & 64.3\% (196) & 60.7\% (84) & 70.0\% (2658) \\
\multicolumn{1}{l|}{} & & & Baseline & 71.8\% (358) & \textbf{74.7\% (1670)} & 73.0\% (196) & \textbf{73.1\% (208)} & \textbf{69.7\% (66)} & \textbf{70.7\% (2858)} \\
\multicolumn{1}{l|}{} & & & Confounded & 70.2\% (530) & 69.9\% (2774) & 73.2\% (410) & 67.6\% (306) & 59.0\% (100) & 68.8\% (4570) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 61.6\% (2028) & 64.7\% (11926) & 62.3\% (1848) & \textbf{64.4\% (1198)} & 59.2\% (424) & 63.7\% (19514) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{61.9\% (2028)} & \textbf{65.0\% (11926)} & 61.2\% (1848) & \textbf{64.4\% (1198)} & \textbf{62.7\% (424)} & 63.6\% (19514) \\
\multicolumn{1}{l|}{} & & & Confounded & 61.6\% (2028) & 64.9\% (11926) & \textbf{63.9\% (1848)} & 63.5\% (1198) & 59.4\% (424) & \textbf{63.9\% (19514)} \\ \hline
\multicolumn{2}{l|}{\multirow{6}{*}{Sex}} & \multirow{3}{*}{0.90} & MUCRAN & 96.0\% (1293) & \textbf{96.8\% (11834)} & \textbf{96.3\% (1789)} & \textbf{96.8\% (2345)} & \textbf{97.2\% (723)} & \textbf{96.1\% (18836)} \\
\multicolumn{2}{l|}{} & & Baseline & 96.1\% (1279) & 94.6\% (11619) & 92.7\% (1716) & 95.5\% (2277) & 95.8\% (689) & 93.7\% (18422) \\
\multicolumn{2}{l|}{} & & Confounded & \textbf{96.5\% (1304)} & 96.0\% (11380) & 95.5\% (1782) & 96.5\% (2335) & 97.2\% (712) & 95.5\% (18327) \\ \cline{3-10} 
\multicolumn{2}{l|}{} & \multirow{3}{*}{0.50} & MUCRAN & \textbf{85.6\% (2789)} & \textbf{85.7\% (24022)} & \textbf{83.9\% (4083)} & 87.2\% (4427) & \textbf{87.4\% (1444)} & \textbf{85.7\% (36765)} \\
\multicolumn{2}{l|}{} & & Baseline & 85.1\% (2789) & 80.1\% (24022) & 79.4\% (4083) & 84.7\% (4427) & 83.4\% (1444) & 81.7\% (36765) \\
\multicolumn{2}{l|}{} & & Confounded & 85.5\% (2789) & 85.2\% (24022) & 83.1\% (4083) & \textbf{87.4\% (4427)} & 86.6\% (1444) & 85.3\% (36765) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> GAN Confounds Article/tables/sites.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[h!]
\caption{Sites for the training set (MGH Pre-2019), as well as the numbers of AD and Controls scanned at each}

\label{tab:sites}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{l|rrrrr}
MRI Site Name  & \multicolumn{1}{l}{No. AD} & \multicolumn{1}{l}{No. CTRL} & \multicolumn{1}{l}{Norm AD (No. AD / Total AD)} & \multicolumn{1}{l}{Norm CTRL (No. CTRL / Total CTRL)} & \multicolumn{1}{l}{Ratio (Norm AD : Norm CTRL)} \\ \hline
MR1WA          & 275                        & 370                          & 0.0653                                          & 0.0293                                                & 2.2243                                          \\
ERMR           & 79                         & 294                          & 0.0188                                          & 0.0233                                                & 0.8041                                          \\
LI\_MR         & 135                        & 779                          & 0.0320                                          & 0.0618                                                & 0.5186                                          \\
LI             & 958                        & 5468                         & 0.2274                                          & 0.4337                                                & 0.5243                                          \\
MR3\_ELL2      & 12                         & 83                           & 0.0028                                          & 0.0066                                                & 0.4327                                          \\
MR1CH          & 196                        & 245                          & 0.0465                                          & 0.0194                                                & 2.3941                                          \\
MR3EL2         & 171                        & 472                          & 0.0406                                          & 0.0374                                                & 1.0842                                          \\
MR1W1          & 246                        & 566                          & 0.0584                                          & 0.0449                                                & 1.3007                                          \\
PR62ELL2       & 34                         & 129                          & 0.0081                                          & 0.0102                                                & 0.7888                                          \\
MRC40168       & 228                        & 294                          & 0.0541                                          & 0.0233                                                & 2.3208                                          \\
MR1A2          & 142                        & 273                          & 0.0337                                          & 0.0217                                                & 1.5566                                          \\
PR67ELL2       & 52                         & 162                          & 0.0123                                          & 0.0128                                                & 0.9606                                          \\
MRFND1         & 228                        & 715                          & 0.0541                                          & 0.0567                                                & 0.9543                                          \\
MR1L6          & 196                        & 98                           & 0.0465                                          & 0.0078                                                & 5.9853                                          \\
MRS1OW         & 74                         & 286                          & 0.0176                                          & 0.0227                                                & 0.7743                                          \\
MR2WA          & 89                         & 98                           & 0.0211                                          & 0.0078                                                & 2.7178                                          \\
MR2EL2         & 94                         & 238                          & 0.0223                                          & 0.0189                                                & 1.1820                                          \\
EXHDMRI        & 21                         & 27                           & 0.0050                                          & 0.0021                                                & 2.3276                                          \\
MR1Y6          & 124                        & 179                          & 0.0294                                          & 0.0142                                                & 2.0731                                          \\
MR2CH          & 149                        & 187                          & 0.0354                                          & 0.0148                                                & 2.3845                                          \\
PR66ELL2       & 36                         & 252                          & 0.0085                                          & 0.0200                                                & 0.4275                                          \\
MR1NS          & 161                        & 192                          & 0.0382                                          & 0.0152                                                & 2.5095                                          \\
PR248          & 44                         & 181                          & 0.0104                                          & 0.0144                                                & 0.7275                                          \\
MRC25157       & 44                         & 64                           & 0.0104                                          & 0.0051                                                & 2.0574                                          \\
MR2Y6          & 160                        & 284                          & 0.0380                                          & 0.0225                                                & 1.6860                                          \\
MR1NY          & 2                          & 12                           & 0.0005                                          & 0.0010                                                & 0.4988                                          \\
MR1EL2         & 131                        & 275                          & 0.0311                                          & 0.0218                                                & 1.4256                                          \\
CHCMRI         & 57                         & 156                          & 0.0135                                          & 0.0124                                                & 1.0935                                          \\
MR3Y6          & 1                          & 3                            & 0.0002                                          & 0.0002                                                & 0.9975                                          \\
MRC20597       & 11                         & 52                           & 0.0026                                          & 0.0041                                                & 0.6331                                          \\
MRC35022       & 28                         & 95                           & 0.0066                                          & 0.0075                                                & 0.8820                                          \\
CHCMR2         & 4                          & 15                           & 0.0009                                          & 0.0012                                                & 0.7980                                          \\
GEMS           & 0                          & 5                            & 0.0000                                          & 0.0004                                                & 0.0000                                          \\
MEDPC          & 9                          & 12                           & 0.0021                                          & 0.0010                                                & 2.2445                                          \\
M247OC0        & 0                          & 1                            & 0.0000                                          & 0.0001                                                & 0.0000                                          \\
BAY4OC         & 2                          & 2                            & 0.0005                                          & 0.0002                                                & 2.9926                                          \\
BAY1OW0        & 0                          & 1                            & 0.0000                                          & 0.0001                                                & 0.0000                                          \\
MR3CH          & 11                         & 16                           & 0.0026                                          & 0.0013                                                & 2.0574                                          \\
BAY3OC         & 0                          & 8                            & 0.0000                                          & 0.0006                                                & 0.0000                                          \\
MR3WA          & 8                          & 16                           & 0.0019                                          & 0.0013                                                & 1.4963                                          \\
MRS3OC0        & 1                          & 2                            & 0.0002                                          & 0.0002                                                & 1.4963                                          \\
MRS5MRS5       & 0                          & 1                            & 0.0000                                          & 0.0001                                                & 0.0000                                          \\
\textbf{TOTAL} & \textbf{4213}              & \textbf{12608}               & \textbf{1.0000}                                 & \textbf{1.0000}                                       & \textbf{}                                      
\end{tabular}
\end{adjustbox}
\end{table}


==> figures/cam_results.tex <==
\begin{figure}[t!]
\centering
%\includegraphics[width=0.30\textwidth]{images/grad_cam_unconfounded.png}
%\includegraphics[width=0.30\textwidth]{images/grad_cam_confounded.png}
{\sffamily
\centering
\includegraphics[width=0.8\textwidth]{images/brain_mesh_perc.png}
}
\caption{\textbf{Averaged gradient class activation map results.} A. Gradient-weighted class activation mapping (Grad-CAM) results for confounded and regressed models, thresholded at 0.15. The regressed model, in which compounding factors were regressed, shows higher activations inside the brain than the confounded model. B. A 3D mesh representation of the Grad-CAM data; a glass brain (in red) is included for visualization purposes. C. Total voxels in each ensemble covering the middle (brain) and edge areas.}
\label{fig:cam_results}
\end{figure}

==> figures/loss.tex <==
\begin{figure}[t!]
\centering
{\sffamily
\includegraphics[width=0.80\textwidth]{images/gan_pipeline_layout.png}

%\begin{tabular}{ccc}
%& \textbf{Regressor} & \textbf{Encoder} \\
%\put(0,0){\rotatebox{90}{\phantom{00000000000000}\textbf{}}}  & \includegraphics[width=0.45\textwidth]{images/encoder_loss.png} & \includegraphics[width=0.45\textwidth]{images/regressor_loss.png}
%\end{tabular}
}

\caption{A. The model used is a CNN that takes a $96\times 96 \times 96$ MRI as input, encodes it to an array of 1024 intermediary features via a CNN and a dense neural network, and regresses these features to an output array. The output array consists of one-hot binary vectors that encode both the primary label (AD/Control) and included confounds (Sex, Age, and so on). B. For training the regressed model, large batches are sampled from an imbalanced dataset such that AD and Control are present in equal proportions. For each training iteration, the model is trained in two-step adversarial process: with the regressor frozen, the encoder is fit to an output array with the label set to its real value, but each confound row set to a constant value ([1,0,0...0]); the regressor is then fit to the array with both the label and its true confound values. C. For testing, labels are predicted through multiple independent models, and their votes are averaged into an ensemble vote. The maximum averaged vote is guaranteed to exceed 0.5, and so that is included in the whole test set; however, a subset of this is also evaluated based on whether or not this averaged vote exceeds a higher threshold. See also Table \ref{tab:results_table}.}
\label{fig:gan_pipeline_fig}
\end{figure}

==> figures/moving_window_auroc.tex <==
\begin{figure}[t!]
\begin{tabular}{cccc}
& \textbf{MGH (post-2019)} & \textbf{BWH} & \textbf{Other} \\
\put(0,0){\rotatebox{90}{\phantom{00000000000}\textbf{}}}  & \includegraphics[width=0.3\textwidth]{images/Ages_mgh.png} & \includegraphics[width=0.3\textwidth]{images/Ages_bwh.png} &
\includegraphics[width=0.3\textwidth]{images/Ages_other.png}
\end{tabular}

\caption{\textbf{}}
\label{fig:confounds_diagram}
\end{figure}

==> figures/test_set_anatomy.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{images/test_anatomy_fig_55.png}

\caption{\textbf{Anatomy of a test set, showing the two critical contributions of this work.} This shows, for Alzheimer's classification, the test set divided into three cases: out-of-distribution data, in which data is too unlike training data to make any determination; indeterminate cases, in which the case may be in-distribution but not be a clear-cut case of Alzheimer's or control; and in-distribution data, in which all models in the ensemble agree on a classification. The age intersection between AD and Control cases show the cases for which MUCRAN performed significantly better than the confounded or baseline comparisons.}
\label{fig:test_set_anatomy}
\end{figure}

==> figures/uncertainty_plots.tex <==
\begin{figure}[t!]
\centering

{\sffamily
\begin{tabular}{ccc}
 \textbf{Confounded} & \textbf{No Confounds} & \textbf{Regressed}\\
 \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_converg_hist_PatientID.png}
 & \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_dud_hist_PatientID.png} &
 \includegraphics[height=0.24\textwidth]{images/AlzStage_institution_all_alexnet_conf_gan_hist_PatientID.png}
\end{tabular} \\
\begin{tabular}{cc}
 \textbf{Distribution Comparison} & \textbf{Accuracy Comparison} \\
 \includegraphics[height=0.36\textwidth]{images/hist_lines_PatientID.png} &
 \includegraphics[height=0.36\textwidth]{images/uncertainty_plots_PatientID.png}
\end{tabular}

}

\caption{\textbf{Accuracies for ensemble predictions with different test set inclusion thresholds.} The histograms show the distribution of values in the regressed (top) and confounded (bottom) ensembles. The graphs show the same data, but explicitly in terms of accuracy, when data below a given threshold is removed. Regressed models offer greater stability and certainty for a larger portion of the data than confounded models.}
\label{fig:uncertainty_plots}
\end{figure}

==> figures/uncertainty_plots2.tex <==
\begin{figure}[h!]
\centering
%\includegraphics[width=0.30\textwidth]{images/grad_cam_unconfounded.png}
%\includegraphics[width=0.30\textwidth]{images/grad_cam_confounded.png}
{\sffamily
\begin{tabular}{cccc}
& \textbf{MGH} & \textbf{BWH} & \textbf{Other} \\
\put(0,0){\rotatebox{90}{\phantom{00000000}\textbf{Before 2019}}}  & {} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_bwh_before_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_other_before_2019.png} \\
\put(0,0){\rotatebox{90}{\phantom{00000000}\textbf{After 2019}}}  & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_mgh_after_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_bwh_after_2019.png} & \includegraphics[width=0.3\textwidth]{images/uncertainty_plots_other_after_2019.png}
\end{tabular}
}
\caption{\textbf{Relative accuracy of each ensemble in threshold values between 0.00 and 0.99.} Lines on these graphs show the intermediate accuracies and number of included datapoints in each test set for values between 0.00 and 0.99; see table \ref{tab:results_table}.}
\label{fig:uncertainty_plots2}
\end{figure}

==> tables/confounds_predictions.tex <==
\begin{table}[b!]
\centering
\caption{Averaged results of the confounds (AUCs) for both the regressed and confounded models.}
\label{tab:confounds_predictions}
\sffamily
\begin{tabular}{lrr}
\toprule
Confound Name &  Confounded Model AUROC & Regressed Model AUROC \\
\midrule
Ages                &    0.644080 &   0.544823 \\
EchoTime            &    0.000000 &   0.000000 \\
Employment Status &    0.568977 &   0.502733 \\
Ethnic Group      &    0.537599 &   0.498418 \\
Imaging Frequency    &    0.790025 &   0.472857 \\
Marital Status   &    0.545788 &   0.507806 \\
Patient Class      &    0.577736 &   0.484328 \\
Pixel Bandwidth      &    0.666692 &   0.493821 \\
Religion         &    0.509234 &   0.488828 \\
Repetition Time      &    0.615542 &   0.486065 \\
Specific Absorption Rate                 &    0.670172 &   0.493353 \\
Sex               &    0.849446 &   0.447886 \\
Slice Thickness      &    0.000000 &   0.000000 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/dataset_description.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\sffamily
\begin{tabular}{l|rr|rr|rr}
\toprule
{} & AD (MGH pre-2019) & Control (MGH pre-2019) & AD (BWH pre-2019) & Control (BWH pre-2019) & AD (Other pre-2019) & CONTROL (Other pre-2019) \\
\midrule
No. Males & 1778 & 5657 & 1810 & 3594 & 221 & 458 \\
No. Females & 2435 & 6951 & 2420 & 5476 & 409 & 848 \\
Age (mean±std) & 722.23 ± 169.55 & 471.82 ± 191.53 & 695.34 ± 172.58 & 504.44 ± 167.14 & 714.34 ± 187.04 & 488.27 ± 166.62 \\
Unique Patient IDs & 1060 & 4215 & 1023 & 2986 & 251 & 520 \\
Slice Thickness & 4.59 ± 0.88 & 4.33 ± 1.04 & 3.93 ± 1.18 & 3.84 ± 1.11 & 3.83 ± 1.49 & 4.11 ± 1.19 \\
No. Unique Datapoints & 4213 & 12608 & 4230 & 9070 & 630 & 1306 \\
No. Unique Sites & 37 & 42 & 38 & 38 & 97 & 211 \\
Echo Time & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 & 0.01 ± 0.01 \\
Repetition Time & 0.55 ± 0.34 & 0.55 ± 0.32 & 0.59 ± 0.29 & 0.59 ± 0.25 & 0.72 ± 0.52 & 0.59 ± 0.36 \\
Specific Absorption Rate & 0.79 ± 0.59 & 0.79 ± 0.64 & 0.72 ± 0.59 & 0.71 ± 0.54 & 0.58 ± 0.49 & 0.70 ± 0.52 \\
Imaging Frequency & 79.71 ± 26.71 & 77.25 ± 25.51 & 81.18 ± 27.55 & 74.34 ± 23.10 & 86.61 ± 29.26 & 81.68 ± 28.06 \\
Pixel Bandwidth & 161.83 ± 77.45 & 149.96 ± 72.58 & 162.42 ± 100.59 & 141.88 ± 71.64 & 201.59 ± 110.49 & 177.18 ± 101.74 \\
No. Unique Religions & 30 & 37 & 30 & 30 & 19 & 27 \\
No. Unique Ethnicities & 5 & 7 & 5 & 7 & 5 & 6 \\
\midrule
{} & AD (MGH post-2019) & Control (MGH post-2019) & AD (BWH post-2019) & Control (BWH post-2019) & AD (Other post-2019) & CONTROL (Other post-2019) \\
\midrule
No. Males & 143 & 529 & 229 & 426 & 58 & 207 \\
No. Females & 211 & 584 & 281 & 595 & 104 & 314 \\
Age (mean±std) & 754.04 ± 176.39 & 552.07 ± 171.99 & 816.87 ± 159.84 & 519.20 ± 186.70 & 794.06 ± 142.25 & 511.45 ± 173.74 \\
Unique Patient IDs & 131 & 461 & 207 & 438 & 84 & 232 \\
Slice Thickness & 4.17 ± 1.30 & 3.92 ± 1.29 & 3.24 ± 1.59 & 2.73 ± 1.51 & 4.24 ± 1.34 & 3.79 ± 1.58 \\
No. Unique Datapoints & 354 & 1113 & 510 & 1021 & 162 & 521 \\
No. Unique Sites & 17 & 18 & 18 & 23 & 30 & 75 \\
Echo Time & 0.02 ± 0.02 & 0.02 ± 0.02 & 0.01 ± 0.00 & 0.01 ± 0.00 & 0.01 ± 0.00 & 0.01 ± 0.00 \\
Repetition Time & 1.06 ± 0.84 & 0.98 ± 0.80 & 0.88 ± 0.64 & 0.93 ± 0.74 & 0.71 ± 0.49 & 0.63 ± 0.50 \\
Specific Absorption Rate & 0.66 ± 0.49 & 0.64 ± 0.50 & 0.37 ± 0.36 & 0.35 ± 0.36 & 0.85 ± 0.54 & 0.80 ± 0.63 \\
Imaging Frequency & 90.58 ± 30.61 & 87.66 ± 30.35 & 99.91 ± 29.37 & 105.22 ± 34.30 & 82.07 ± 27.54 & 80.00 ± 26.68 \\
Pixel Bandwidth & 249.56 ± 102.89 & 236.10 ± 110.17 & 253.09 ± 109.79 & 258.53 ± 102.76 & 171.41 ± 92.82 & 161.73 ± 77.02 \\
No. Unique Religions & 21 & 25 & 21 & 24 & 12 & 14 \\
No. Unique Ethnicities & 5 & 6 & 3 & 5 & 3 & 5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Statistics associated with the three datasets used. The model in this paper was trained on the pre-2019 MGH data. Shown for continuous values are the mean and standard deviations. \label{tab:dataset_description}}
\end{table}

==> tables/results_alz.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results on Alzheimer's classification when the whole test set is included (threshold = 0.5), and results, on five test sets and the combined test sets, for which the averaged prediction in its respective category is above 0.90 (i.e., each model in the ensemble unanimously agrees). Shown are the accuracies on the portion of the dataset included after thresholding, and the size of that test set (in parentheses). Included as well are age-matched samples. See also Figure \ref{fig:gan_pipeline_fig}C.}

\label{tab:results_alz}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{l|}{\multirow{12}{*}{Alzheimer’s}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{92.5\% (548)} & \textbf{89.2\% (3721)} & \textbf{93.5\% (367)} & \textbf{92.1\% (643)} & \textbf{90.5\% (285)} & \textbf{89.1\% (5783)} \\
\multicolumn{1}{l|}{} & & & Baseline & 87.7\% (778) & 84.4\% (6198) & 89.8\% (637) & 88.4\% (976) & 91.0\% (390) & 84.7\% (9469) \\
\multicolumn{1}{l|}{} & & & Confounded & 89.5\% (829) & 84.1\% (7265) & 87.6\% (740) & 86.3\% (1138) & 90.5\% (419) & 83.9\% (10951) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 75.8\% (1463) & 72.4\% (13303) & 75.2\% (1531) & \textbf{76.9\% (1936)} & 80.2\% (681) & 72.1\% (20857) \\
\multicolumn{1}{l|}{} & & & Baseline & 77.4\% (1463) & \textbf{72.9\% (13303)} & \textbf{76.3\% (1531)} & 74.7\% (1936) & \textbf{81.6\% (681)} & \textbf{72.4\% (20857)} \\
\multicolumn{1}{l|}{} & & & Confounded & \textbf{78.4\% (1463)} & \textbf{72.9\% (13303)} & 74.7\% (1531) & 74.7\% (1936) & 81.2\% (681) & 72.3\% (20857) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Age-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{86.0\% (150)} & \textbf{67.0\% (880)} & \textbf{77.3\% (44)} & \textbf{73.5\% (166)} & \textbf{71.9\% (32)} & \textbf{70.1\% (1516)} \\
\multicolumn{1}{l|}{} & & & Baseline & 71.6\% (222) & 57.7\% (1962) & 66.4\% (110) & 65.3\% (314) & 65.8\% (76) & 60.8\% (3064) \\
\multicolumn{1}{l|}{} & & & Confounded & 71.1\% (228) & 54.6\% (2452) & 59.1\% (164) & 60.1\% (376) & 54.3\% (70) & 56.6\% (3846) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & \textbf{65.2\% (494)} & \textbf{56.7\% (6372)} & 55.6\% (446) & \textbf{60.7\% (746)} & \textbf{66.7\% (168)} & \textbf{58.3\% (10264)} \\
\multicolumn{1}{l|}{} & & & Baseline & 64.8\% (494) & 56.6\% (6372) & \textbf{57.8\% (446)} & 57.1\% (746) & 65.5\% (168) & 57.6\% (10264) \\
\multicolumn{1}{l|}{} & & & Confounded & 64.2\% (494) & 55.2\% (6372) & 55.2\% (446) & 55.9\% (746) & 59.5\% (168) & 56.7\% (10264) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/results_local.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results for localized anomaly classifications, as well as a site-matched sample.}

\label{tab:results_local}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{p{2cm}|}{\multirow{12}{*}{\parbox{2cm}{Ischemia/ Lesion/ Tumor/ Head Trauma}}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & 74.9\% (521) & 80.5\% (2918) & 65.1\% (763) & 65.8\% (803) & 59.4\% (229) & 75.9\% (6783) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{76.2\% (564)} & \textbf{82.3\% (3452)} & \textbf{71.5\% (820)} & \textbf{72.9\% (893)} & \textbf{71.8\% (252)} & \textbf{79.5\% (7891)} \\
\multicolumn{1}{l|}{} & & & Confounded & 73.6\% (754) & 78.8\% (5177) & 66.8\% (1025) & 67.1\% (1217) & 64.3\% (367) & 75.3\% (10500) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 63.2\% (2421) & 68.1\% (19786) & 61.1\% (3558) & 62.5\% (3780) & 62.6\% (1276) & 66.2\% (35264) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{63.9\% (2421)} & \textbf{68.7\% (19786)} & \textbf{61.7\% (3558)} & \textbf{64.5\% (3780)} & \textbf{62.7\% (1276)} & \textbf{67.1\% (35264)} \\
\multicolumn{1}{l|}{} & & & Confounded & 63.5\% (2421) & 68.4\% (19786) & 60.5\% (3558) & 62.1\% (3780) & 60.7\% (1276) & 66.1\% (35264) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Site-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{72.3\% (368)} & 71.8\% (1486) & \textbf{74.4\% (238)} & 64.3\% (196) & 60.7\% (84) & 70.0\% (2658) \\
\multicolumn{1}{l|}{} & & & Baseline & 71.8\% (358) & \textbf{74.7\% (1670)} & 73.0\% (196) & \textbf{73.1\% (208)} & \textbf{69.7\% (66)} & \textbf{70.7\% (2858)} \\
\multicolumn{1}{l|}{} & & & Confounded & 70.2\% (530) & 69.9\% (2774) & 73.2\% (410) & 67.6\% (306) & 59.0\% (100) & 68.8\% (4570) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 61.6\% (2028) & 64.7\% (11926) & 62.3\% (1848) & \textbf{64.4\% (1198)} & 59.2\% (424) & 63.7\% (19514) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{61.9\% (2028)} & \textbf{65.0\% (11926)} & 61.2\% (1848) & \textbf{64.4\% (1198)} & \textbf{62.7\% (424)} & 63.6\% (19514) \\
\multicolumn{1}{l|}{} & & & Confounded & 61.6\% (2028) & 64.9\% (11926) & \textbf{63.9\% (1848)} & 63.5\% (1198) & 59.4\% (424) & \textbf{63.9\% (19514)} \end{tabular}
\end{adjustbox}
\end{table}


==> tables/results_table.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t]
\caption{Results when the whole test set is included, and results for which the averaged prediction in its respective category is above 0.99 (i.e., each model in the ensemble unanimously agrees).}

\label{tab:results_table}
\sffamily
\begin{tabular}{rllrrrrr}
\toprule
\multirow{2}{*}{Threshold} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{MGH} & \multicolumn{2}{c|}{BWH} & \multicolumn{2}{c|}{Others} \\
 & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} \\ \hline
0.99 & \multirow{2}{*}{Regressed} & Accuracy & 92.2 & 86.3 & 91.5 & 89.5 & 95.2 \\
 & & No. Included Datapoints & 628 & 5297 & 539 & 848 & 335 \\
 & \multirow{2}{*}{Confounded} & Accuracy & 88.8 & 85.5 & 90.0 & 88.0 & 92.1 \\
 & & No. Included Datapoints & 760 & 6565 & 671 & 1031 & 382 \\
 & \multirow{2}{*}{Label Only} & Accuracy & 89.3 & 84.2 & 88.8 & 86.3 & 92.6 \\
 & & No. Included Datapoints & 836 & 6829 & 695 & 1065 & 417 \\ \hline
0.50 & \multirow{2}{*}{Regressed} & Accuracy & 76.2 & 73.2 & 75.8 & 75.7 & 81.2 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
 & \multirow{2}{*}{Confounded} & Accuracy & 78.5 & 73.4 & 75.2 & 75.9 & 82.5 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
 & \multirow{2}{*}{Label Only} & Accuracy & 78.9 & 72.7 & 75.0 & 75.2 & 81.6 \\
 & & No. Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/results_table_unthresholded.tex <==
\begin{table}[]
\caption{Results when all data are included (i.e., no threshold).}
\label{tab:results_table_unthresholded}
\begin{tabular}{lllllll}
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{MGH} & \multicolumn{2}{c|}{BWH} & \multicolumn{2}{c|}{Others} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} \\ \hline
\multirow{2}{*}{Regressed} & Accuracy & 76.2 & 73.2 & 75.8 & 75.7 & 81.2 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\multirow{2}{*}{Confounded} & Accuracy & 78.5 & 73.4 & 75.2 & 75.9 & 82.5 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 \\
\multirow{2}{*}{No confounds} & Accuracy & 78.9 & 72.7 & 75.0 & 75.2 & 81.6 \\
 & \# Included Datapoints & 1467 & 13300 & 1531 & 1936 & 683 
\end{tabular}
\end{table}

==> tables/results_tablev2.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t]
\caption{Results when the whole test set is included, and results for which the averaged prediction in its respective category is above 0.99 (i.e., each model in the ensemble unanimously agrees).}

\label{tab:results_table}
\sffamily
\begin{tabular}{lllllll|l}
\multirow{2}{*}{Threshold} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{MGH}       & \multicolumn{2}{c|}{BWH}                                       & \multicolumn{2}{c|}{Others}                      & \multicolumn{1}{l|}{\textbf{All}} \\
                           & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019        & \multicolumn{1}{l|}{\textbf{}}    \\ \hline
0.99                       & Regressed                                    & 92.2\% (628/1467)              & 86.3\% (5297/13300)           & 91.5\% (539/1531)              & 89.5\% (848/1936)             & 95.2\% (335/683) & \textbf{86.9\% (7958/20860)}      \\
                           & Confounded                                   & 88.8\% (760/1467)              & 85.5\% (6565/13300)           & 90.0\% (671/1531)              & 88.0\% (1031/1936)            & 92.1\% (382/683) & \textbf{85.3\% (9892/20860)}      \\
                           & Label only                                   & 89.3\% (836/1467)              & 84.2\% (6829/13300)           & 88.8\% (695/1531)              & 86.3\% (1065/1936)            & 92.6\% (417/683) & \textbf{84.3\% (10374/20860)}     \\ \hline
0.00                       & Regressed                                    & 76.2\% (1467/1467)             & 73.2\% (13300/13300)          & 75.8\% (1531/1531)             & 75.7\% (1936/1936)            & 81.2\% (683/683) & \textbf{72.7\% (20860/20860)}     \\
                           & Confounded                                   & 78.5\% (1467/1467)             & 73.4\% (13300/13300)          & 75.2\% (1531/1531)             & 75.9\% (1936/1936)            & 82.5\% (683/683) & \textbf{72.8\% (20860/20860)}     \\
                           & Label only                                   & 78.9\% (1467/1467)             & 72.7\% (13300/13300)          & 75.0\% (1531/1531)             & 75.2\% (1936/1936)            & 81.6\% (683/683) & \textbf{72.3\% (20860/20860)}    
\end{tabular}

\end{table}


==> tables/results_tablev3.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht]
\caption{Results when the whole test set is included (threshold = 0.5), and results for which the averaged prediction in its respective category is above 0.90 (i.e., each model in the ensemble unanimously agrees). Shown are the accuracies on the portion of the dataset included after thresholding, and the size of that test set (in parentheses). Included as well are age-matched samples of the Alzheimer's classification and site-matched samples of localized anomaly classifications. See also Figure \ref{fig:gan_pipeline_fig} C.}

\label{tab:results_table}
\sffamily
\centering
\begin{adjustbox}{width=0.90\textwidth,totalheight=0.80\textheight,keepaspectratio}
\begin{tabular}{p{2cm}p{2cm}|l|l|lllll|l}
\multicolumn{2}{l|}{\multirow{2}{*}{Classification task}} & \multirow{2}{*}{\parbox{2cm}{Uncertainty Threshold}} & \multirow{2}{*}{Model} & \multicolumn{1}{l|}{MGH} & \multicolumn{2}{l|}{BWH} & \multicolumn{2}{l|}{Others} & \multirow{2}{*}{All} \\
\multicolumn{2}{l|}{} & & & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & \multicolumn{1}{l|}{Post-2019} & \multicolumn{1}{l|}{Pre-2019} & Post-2019 & \\ \hline
\multicolumn{1}{l|}{\multirow{12}{*}{Alzheimer’s}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{92.5\% (548)} & \textbf{89.2\% (3721)} & \textbf{93.5\% (367)} & \textbf{92.1\% (643)} & \textbf{90.5\% (285)} & \textbf{89.1\% (5783)} \\
\multicolumn{1}{l|}{} & & & Baseline & 87.7\% (778) & 84.4\% (6198) & 89.8\% (637) & 88.4\% (976) & 91.0\% (390) & 84.7\% (9469) \\
\multicolumn{1}{l|}{} & & & Confounded & 89.5\% (829) & 84.1\% (7265) & 87.6\% (740) & 86.3\% (1138) & 90.5\% (419) & 83.9\% (10951) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 75.8\% (1463) & 72.4\% (13303) & 75.2\% (1531) & \textbf{76.9\% (1936)} & 80.2\% (681) & 72.1\% (20857) \\
\multicolumn{1}{l|}{} & & & Baseline & 77.4\% (1463) & \textbf{72.9\% (13303)} & \textbf{76.3\% (1531)} & 74.7\% (1936) & \textbf{81.6\% (681)} & \textbf{72.4\% (20857)} \\
\multicolumn{1}{l|}{} & & & Confounded & \textbf{78.4\% (1463)} & \textbf{72.9\% (13303)} & 74.7\% (1531) & 74.7\% (1936) & 81.2\% (681) & 72.3\% (20857) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Age-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{86.0\% (150)} & \textbf{67.0\% (880)} & \textbf{77.3\% (44)} & \textbf{73.5\% (166)} & \textbf{71.9\% (32)} & \textbf{70.1\% (1516)} \\
\multicolumn{1}{l|}{} & & & Baseline & 71.6\% (222) & 57.7\% (1962) & 66.4\% (110) & 65.3\% (314) & 65.8\% (76) & 60.8\% (3064) \\
\multicolumn{1}{l|}{} & & & Confounded & 71.1\% (228) & 54.6\% (2452) & 59.1\% (164) & 60.1\% (376) & 54.3\% (70) & 56.6\% (3846) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & \textbf{65.2\% (494)} & \textbf{56.7\% (6372)} & 55.6\% (446) & \textbf{60.7\% (746)} & \textbf{66.7\% (168)} & \textbf{58.3\% (10264)} \\
\multicolumn{1}{l|}{} & & & Baseline & 64.8\% (494) & 56.6\% (6372) & \textbf{57.8\% (446)} & 57.1\% (746) & 65.5\% (168) & 57.6\% (10264) \\
\multicolumn{1}{l|}{} & & & Confounded & 64.2\% (494) & 55.2\% (6372) & 55.2\% (446) & 55.9\% (746) & 59.5\% (168) & 56.7\% (10264) \\ \hline
\multicolumn{1}{p{2cm}|}{\multirow{12}{*}{\parbox{2cm}{Ischemia/ Lesion/ Tumor/ Head Trauma}}} & \multirow{6}{*}{All} & \multirow{3}{*}{0.90} & MUCRAN & 74.9\% (521) & 80.5\% (2918) & 65.1\% (763) & 65.8\% (803) & \textbf{59.4\% (229)} & 75.9\% (6783) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{76.2\% (564)} & \textbf{82.3\% (3452)} & \textbf{71.5\% (820)} & \textbf{72.9\% (893)} & \textbf{71.8\% (252)} & \textbf{79.5\% (7891)} \\
\multicolumn{1}{l|}{} & & & Confounded & 73.6\% (754) & 78.8\% (5177) & 66.8\% (1025) & 67.1\% (1217) & 64.3\% (367) & 75.3\% (10500) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 63.2\% (2421) & 68.1\% (19786) & 61.1\% (3558) & 62.5\% (3780) & 62.6\% (1276) & 66.2\% (35264) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{63.9\% (2421)} & \textbf{68.7\% (19786)} & \textbf{61.7\% (3558)} & \textbf{64.5\% (3780)} & \textbf{62.7\% (1276)} & \textbf{67.1\% (35264)} \\
\multicolumn{1}{l|}{} & & & Confounded & 63.5\% (2421) & 68.4\% (19786) & 60.5\% (3558) & 62.1\% (3780) & 60.7\% (1276) & 66.1\% (35264) \\ \cline{2-10} 
\multicolumn{1}{l|}{} & \multirow{6}{*}{\parbox{2cm}{Site-matched sample}} & \multirow{3}{*}{0.90} & MUCRAN & \textbf{72.3\% (368)} & 71.8\% (1486) & \textbf{74.4\% (238)} & 64.3\% (196) & 60.7\% (84) & 70.0\% (2658) \\
\multicolumn{1}{l|}{} & & & Baseline & 71.8\% (358) & \textbf{74.7\% (1670)} & 73.0\% (196) & \textbf{73.1\% (208)} & \textbf{69.7\% (66)} & \textbf{70.7\% (2858)} \\
\multicolumn{1}{l|}{} & & & Confounded & 70.2\% (530) & 69.9\% (2774) & 73.2\% (410) & 67.6\% (306) & 59.0\% (100) & 68.8\% (4570) \\ \cline{3-10} 
\multicolumn{1}{l|}{} & & \multirow{3}{*}{0.50} & MUCRAN & 61.6\% (2028) & 64.7\% (11926) & 62.3\% (1848) & \textbf{64.4\% (1198)} & 59.2\% (424) & 63.7\% (19514) \\
\multicolumn{1}{l|}{} & & & Baseline & \textbf{61.9\% (2028)} & \textbf{65.0\% (11926)} & 61.2\% (1848) & \textbf{64.4\% (1198)} & \textbf{62.7\% (424)} & 63.6\% (19514) \\
\multicolumn{1}{l|}{} & & & Confounded & 61.6\% (2028) & 64.9\% (11926) & \textbf{63.9\% (1848)} & 63.5\% (1198) & 59.4\% (424) & \textbf{63.9\% (19514)} \\ \hline
\multicolumn{2}{l|}{\multirow{6}{*}{Sex}} & \multirow{3}{*}{0.90} & MUCRAN & 96.0\% (1293) & \textbf{96.8\% (11834)} & \textbf{96.3\% (1789)} & \textbf{96.8\% (2345)} & \textbf{97.2\% (723)} & \textbf{96.1\% (18836)} \\
\multicolumn{2}{l|}{} & & Baseline & 96.1\% (1279) & 94.6\% (11619) & 92.7\% (1716) & 95.5\% (2277) & 95.8\% (689) & 93.7\% (18422) \\
\multicolumn{2}{l|}{} & & Confounded & \textbf{96.5\% (1304)} & 96.0\% (11380) & 95.5\% (1782) & 96.5\% (2335) & 97.2\% (712) & 95.5\% (18327) \\ \cline{3-10} 
\multicolumn{2}{l|}{} & \multirow{3}{*}{0.50} & MUCRAN & \textbf{85.6\% (2789)} & \textbf{85.7\% (24022)} & \textbf{83.9\% (4083)} & 87.2\% (4427) & \textbf{87.4\% (1444)} & \textbf{85.7\% (36765)} \\
\multicolumn{2}{l|}{} & & Baseline & 85.1\% (2789) & 80.1\% (24022) & 79.4\% (4083) & 84.7\% (4427) & 83.4\% (1444) & 81.7\% (36765) \\
\multicolumn{2}{l|}{} & & Confounded & 85.5\% (2789) & 85.2\% (24022) & 83.1\% (4083) & \textbf{87.4\% (4427)} & 86.6\% (1444) & 85.3\% (36765) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

